Unconstraining Multi-Robot Manipulation: Enabling Arbitrary Constraints in ECBS with Bounded Sub-Optimality

Multi-Robot-Arm Motion Planning (M-RAMP) is a challenging problem featuring complex single-agent planning and multi-agent coordination. Recent advancements in extending the popular Conflict-Based Search (CBS) algorithm have made large strides in solving Multi-Agent Path Finding (MAPF) problems. However, fundamental challenges remain in applying CBS to M-RAMP. A core challenge is the existing reliance of the CBS framework on conservative "complete" constraints. These constraints ensure solution guarantees but often result in slow pruning of the search space -- causing repeated expensive single-agent planning calls. Therefore, even though it is possible to leverage domain knowledge and design incomplete M-RAMP-specific CBS constraints to more efficiently prune the search, using these constraints would render the algorithm itself incomplete. This forces practitioners to choose between efficiency and completeness. In light of these challenges, we propose a novel algorithm, Generalized ECBS, aimed at removing the burden of choice between completeness and efficiency in MAPF algorithms. Our approach enables the use of arbitrary constraints in conflict-based algorithms while preserving completeness and bounding sub-optimality. This enables practitioners to capitalize on the benefits of arbitrary constraints and opens a new space for constraint design in MAPF that has not been explored. We provide a theoretical analysis of our algorithms, propose new "incomplete" constraints, and demonstrate their effectiveness through experiments in M-RAMP.

==> figure_experiments_incomplete.tex <==
\begin{figure*}[t]
  \begin{minipage}{0.64\textwidth}
    \centering
    \begin{subfigure}{\linewidth}
      % \includegraphics[height=4.5cm]{figures/robots/mramp_rack_square.png}
        SPHERE CONSTRAINT
      \hspace{0.3cm}
      SPHERE XL CONSTRAINT
      % \includegraphics[height=4.6cm, width=6.2cm]{figures/experiments/confusion_matrix_eight_time.png}
    %   \caption{}
    \end{subfigure}
    % Add a table.
    % \caption{Images in the first row}
  \end{minipage}
\hspace{-0.5cm}
\begin{minipage}{0.36\textwidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|}
\hline
8 Robots & \cellcolor[HTML]{C0C0C0}Success & \cellcolor[HTML]{C0C0C0} Timeout (\%) & \cellcolor[HTML]{C0C0C0} Failure (\%) \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \cellcolor[HTML]{C0C0C0}ECBS & 40\% & \cellcolor[HTML]{EFEFEF}\ 60\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS & 48\% & 52\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-P & 78\% & 22\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-A & 78\% & 22\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-S & 76\% & 24\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-LS & 10\% & 10\% & 80\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-XLS & 4\% & 10\% & 86\% \\ \hline
\end{tabular}
}
\end{minipage}

\hspace{0.2cm}

\begin{minipage}{0.64\textwidth}
\centering
\begin{subfigure}{\linewidth}
  % \includegraphics[width=4.5cm]{figures/robots/panda_four_binpick_square.png}
  PRIORITY CONSTRAINT
  \hspace{0.3cm}
  AVOIDANCE CONSTRAINT
  % \includegraphics[height=4.6cm, width=6.2cm]{figures/experiments/confusion_matrix_four_time.png}
%   \caption{}
\end{subfigure}
% Add a table.
% \caption{Images in the first row}
\end{minipage}
\hspace{-0.5cm}
\begin{minipage}{0.36\textwidth}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|}
\hline
4 Robots & \cellcolor[HTML]{C0C0C0}Success & \cellcolor[HTML]{C0C0C0} Timeout (\%) & \cellcolor[HTML]{C0C0C0} Failure (\%) \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \cellcolor[HTML]{C0C0C0}ECBS & 40\% & \cellcolor[HTML]{EFEFEF}\ 60\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS & 86\% & 14\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-P & 98\% & 2\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-A & 98\% & 2\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-S & 96\% & 4\% & 0\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-LS & 62\% & 4\% & 34\% \\ \hline
\cellcolor[HTML]{C0C0C0}ECBS-XLS & 62\% & 2\% & 36\% \\ \hline
\end{tabular}
}
\end{minipage}
  
  \caption{{\color{red}A figure showing the effects of directly using \textbf{incomplete constraints \textbf{instead} of the regular constraints} in ECBS. This shows potentially significant improvements with some failures attributed to timeout and other failures attributed to planning failure (incompleteness). Table for 4 robots, table for 8 robots, reference the images in the next figure for visualization.}}
  \label{fig:experimental_incomplete}
\end{figure*}
